STCN: Stochastic Temporal Convolutional Networks

Convolutional architectures have recently been shown to be competitive on many sequence modelling tasks when compared to the de-facto standard of recurrent neural networks (RNNs), while providing computational and modeling advantages due to inherent parallelism. However, currently there remains a performance gap to more expressive stochastic RNN variants, especially those with several layers of dependent random variables. In this work, we propose stochastic temporal convolutional networks (STCNs), a novel architecture that combines the computational advantages of temporal convolutional networks (TCN) with the representational power and robustness of stochastic latent spaces. In particular, we propose a hierarchy of stochastic latent variables that captures temporal dependencies at different time-scales. The architecture is modular and flexible due to the decoupling of the deterministic and stochastic layers. We show that the proposed architecture achieves state of the art log-likelihoods across several tasks. Finally, the model is capable of predicting high-quality synthetic samples over a long-range temporal horizon in modeling of handwritten text.

==> Makefile <==
BUILD=build/

all: iclr2019_stcn.pdf

watch:
	@while true; do\
		inotifywait -e modify *.tex **/*.tex; \
		make; \
	done

%.pdf: %.tex $(wildcard **/*.tex)
	@if [ ! -d $(BUILD) ]; then \
		mkdir $(BUILD); \
	fi
	@latexmk -jobname=$(BUILD)$(basename $@) \
		-latexoption="-shell-escape" \
		-pdf $<
	@cp build/$@ $@

clean:
	@if [ -d $(BUILD) ]; then \
		rm -rf $(BUILD); \
		echo "rm -rf $(BUILD)"; \
	fi
	rm 1083.pdf 1083-supp.pdf


==> sec/05_evaluation.tex <==
% !TEX root = ../iclr2019_stcn.tex

\section{Qualitative Evaluation}\label{sec:evaluation}
TODO

==> sec/07_tables.tex <==
% !TEX root = ../iclr2019_stcn.tex

\section{Tables From Manuel}

%% ALL TABLES COMBINED

\iffalse
%% TIMIT AND IAMONDB ONLY
\begin{table}
\centering
\begin{tabular}{l||c|c|c|c}
  \hline
  \multicolumn{1}{l||}{\multirow{2}{*}{Models} } & \multicolumn{2}{c|}{TIMIT} & \multicolumn{2}{c}{Iamondb}\\
  \cline{2-5}  
  & Gaussian & GMM & Gaussian & GMM \\
  \hline
  \hline
  Wavenet $^\ast$ & -7443 & 30188 & 1053 & 1381\\
  \hline
  Wavenet-dense & -8579 & 30636 & 1030 & 1380\\
  \hline  
  RNN \cite{chung2015recurrent} & -1900 & 26643 & 1016 & 1358\\
  \hline
  VRNN \cite{chung2015recurrent} & $\geq$ 28805 & $\geq$ 28982 & $\geq$ 1337 & $\geq$ 1384\\
  \hline
  \modelname & $\geq$ 36553 & $\geq$ 32588 & $\geq$ 1308 & TBD\\
  \hline
  \modelnameskip & $\geq$ 38450 & $\geq$ 34567 & $\geq$ 1685 & TBD\\
  \hline
  \modelname $+$ kla & $\geq$ \textbf{48066} & $\geq$ \textbf{45063} & $\geq$ 1362 & TBD\\
  \hline
  \modelnameskip $+$ kla & $\geq$ 43540 & $\geq$ 42591 & $\geq$ 1714 & TBD\\
  \hline
  \hline
  Z-forcing \cite{goyal2017z} & $\geq$ 70469 & n/a & n/a & n/a\\
  \hline
  SRNN \cite{fraccaro2016sequential} & 60550 & n/a & n/a & n/a\\
  \hline
\end{tabular}
\caption{Performance on TIMIT and Iamondb. A star $^\ast$ denotes own implementation of model.}
\label{tab:timit_iamondb}
\end{table}


%% DEEPWRITING ONLY
\begin{table}
\centering
\begin{tabular}{l||c|c}
  \hline
  \multicolumn{1}{l||}{\multirow{2}{*}{Models} } & \multicolumn{2}{c}{Deepwriting} \\
  \cline{2-3}  
  & Gaussian & GMM \\
  \hline
  \hline
  Wavenet $^\ast$ & 1.21 & 2.34\\
  \hline
  Wavenet-dense & 1.19 & 2.47\\
  \hline  
  RNN $^\ast$ & 1.34 & 1.98\\
  \hline
  VRNN $^\ast$ & $\geq$ 1.84 & $\geq$ 2.57\\
  \hline
  \modelname & $\geq$ 1.79 & $\geq$ 2.38\\
  \hline
  \modelnameskip & $\geq$ \textbf{2.44} & $\geq$ \textbf{2.66}\\
  \hline
  \modelname $+$ kla & $\geq$ 1.71 & TBD \\
  \hline
  \modelnameskip $+$ kla & $\geq$ 2.27 & TBD\\
  \hline
\end{tabular}
\caption{Performance on Deepwriting dataset. A star $^\ast$ denotes own implementation of model.}
\label{tab:deepwriting}
\end{table}

\fi
%% MNIST ONLY

